Self-hybridized vibrational-Mie polaritons in water droplets

We study the self-hybridization between Mie modes supported by water droplets with stretching and bending vibrations in water molecules. Droplets with radii $>2.7~\mu m$ are found to be polaritonic on the onset of the ultrastrong light-matter coupling regime. Similarly, the effect is observed in larger deuterated water droplets at lower frequencies. Our results indicate that polaritonic states are ubiquitous in nature and occur in water droplets in mists, fogs, and clouds. This finding may have implications not only for polaritonic physics but also for aerosol and atmospheric sciences.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

